The MBTA Pipeline for Detecting Compact Binary Coalescences in the Fourth LIGO-Virgo-KAGRA Observing Run

In this paper, we describe the Multi-Band Template Analysis (MBTA) search pipeline dedicated to the detection of compact binary coalescence (CBC) gravitational wave signals from the data obtained by the LIGO-Virgo-KAGRA collaboration (LVK) during the fourth observing run (O4), which started in May 2023. We give details on the configuration of the pipeline and its evolution compared to the third observing run (O3). We focus here on the configuration used for the offline results of the first part of the run (O4a), which are part of the GWTC-4 catalog (in preparation). We also give a brief summary of the online configuration and highlight some of the changes implemented or considered for the second part of O4 (O4b).

==> 00-preamble.tex <==
\usepackage[top=2cm,bottom=2cm,right=2cm,left=2cm]{geometry}
\usepackage[utf8]{inputenc}
\usepackage{graphicx} % Required for inserting images
\usepackage[usenames, dvipsnames]{color}  % Coloured text etc.
\usepackage[usenames, dvipsnames]{xcolor}  % Coloured text etc.
\usepackage{soul}
\usepackage{siunitx}
\usepackage{hyperref}
%\usepackage{natbib}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{multirow}
\usepackage{multicol}
\usepackage{printlen}
\usepackage{makecell}
\usepackage{xspace}
\usepackage[skins]{tcolorbox}
\tcbuselibrary{breakable}
\usepackage[switch]{lineno}
\usepackage{sectsty}
\usepackage{authblk}
\usepackage[toc,page]{appendix}
\usepackage{csquotes}
\usepackage{cite}

\renewcommand\Affilfont{\itshape\small}

\DeclareRobustCommand{\pending}[1]{{\sethlcolor{lightgray}\hl{#1}}}
\DeclareRobustCommand{\refnec}{{\sethlcolor{Red}\hl{REF NEEDED}}}
\newcommand{\hiddencomment}[1]{}

\tcbset{commonstyle/.style={boxrule=0pt,sharp corners,enhanced jigsaw,nobeforeafter,boxsep=0pt,left=\fboxsep,right=\fboxsep,enforce breakable}}
\newtcolorbox{mycolorbox}[1][]{commonstyle,#1}

\colorlet{soulSkyBlue}{SkyBlue!10}
\colorlet{soulRubineRed}{RubineRed!10}
\newcommand{\boilerplate}[1]{\begin{mycolorbox}[colback=soulSkyBlue]#1\end{mycolorbox}}
\newcommand{\newstuff}[1]{\begin{mycolorbox}[colback=soulRubineRed]#1\end{mycolorbox}}


\newcommand{\lvk}{LIGO-Virgo-KAGRA collaboration}
\newcommand{\pastro}{\ensuremath{p_\text{astro}}\xspace}
\newcommand{\pbns}{\ensuremath{p_\text{BNS}}\xspace}
\newcommand{\pbbh}{\ensuremath{p_\text{BBH}}\xspace}
\newcommand{\pnsbh}{\ensuremath{p_\text{NSBH}}\xspace}
\newcommand{\pterr}{\ensuremath{p_\text{terr}}\xspace}
\newcommand{\psource}{\ensuremath{p_\text{source}}\xspace}
\newcommand{\Msun}{\ensuremath{\mathrm{M_{\odot}}}\xspace}
\newcommand{\mchirp}{\ensuremath{m_{\text{chirp}}}\xspace}
\newcommand{\mtot}{\ensuremath{m_{\text{tot}}}\xspace}
\newcommand{\mchirptot}{\ensuremath{m_{\text{chirp/tot}}}\xspace}
\newcommand{\spineff}{\ensuremath{\chi_\mathrm{eff}}\xspace}

\newcommand{\gracedb}{\texttt{GraceDB} }
\newcommand{\snrexcess}{\ensuremath{\mathrm{SNR}\mbox{-}\mathrm{Excess}}\xspace}

\renewcommand\cellgape{\Gape[3pt]}

